Properties of low angular momentum general relativistic MHD accretion flows around black holes

In this proceeding, we provide a novel approach to study the General Relativistic Magnetohydrodynamic (GRMHD) accretion flows around rotating black holes (BHs). In doing so, we choose a sub-Keplerian distribution of angular momentum of the flow, which is necessary for the accreting matter to reach the event horizon of the BH. Further, we consider the convergent flow to be confined about the disk mid-plane and is threaded by both radial ($b^r$) and toroidal ($b^\phi$) magnetic field components. For simplicity, we neglect any motion along the vertical ($\theta$) direction, maintaining a vertical (hydrostatic) equilibrium about the midplane. With this, we describe the family of multi-trans-magnetosonic accretion solutions around rotating BHs and examine how the conserved magnetic flux ($\Phi$) and BH spin ($a_{\rm k}$) affect the accretion flow properties. Finally, we provide an insight into the thermal emissions from the magnetized disk for a specific set of accretion solutions.

==> organizers.tex <==
%to switch ON running title
%\markboth{Organizing committees}{Organizing committees}

\wstoc{Organizing committees}{}

\title{Organizing committees}

\begin{center}
{\bf Series editorial board}\\
{\it for the series on advances in quantum many-body theory}
\end{center}
\vspace*{1em}

\begin{tabular}{ll}
R. F. Bishop (Chairman) & -- UMIST, Manchester, UK\\
C. E. Campbell & -- University of Minnesota, USA \\
J. W. Clark & -- Washington University, St.\ Louis, USA \\
S. Fantoni & -- SISSA, Trieste, Italy
\end{tabular}

\vspace*{0.12in}

\noindent
\begin{center}
{\bf International advisory committee}\\
{\it for the Series of International Conferences on}\\
{\it Recent Progress in Many-Body Theories}
\end{center}
\vspace*{1em}

\noindent
\begin{tabular}{ll}
R. F. Bishop (Chairman) & -- UMIST, Manchester, UK\\
S. Fantoni (Secretary) & -- SISSA, Trieste, Italy\\
C. E. Campbell (Treasurer) & -- University of Minnesota, USA\\
H. K\"{u}mmel (Hon.\ President) & -- Ruhr-Universit\"{a}t
Bochum, Germany \\
J. A. Carlson & -- Los Alamos National Laboratory, USA \\
S. A. Chin & -- Texas A \& M University, USA \\
J. W. Clark & -- Washington University, St.~Louis, USA \\
P. Fulde & -- Max-Planck-Institut f\"{u}r Komplexer  \\
& ~~~Systeme, Dresden, Germany\\
A. Kallio & -- University of Oulu, Finland \\
E. Krotscheck & -- Johannes Universit\"{a}t Linz, Austria \\
C. Lhuillier & -- Universit\'{e} Pierre et Marie Curie, Paris\\
A. MacDonald & -- Indiana University, Bloomington, USA \\
E. Manousakis & -- Florida State University, USA \\
D. Neilson & -- University of New South Wales, Sydney, \\
& ~~~Australia \\
M. L. Ristig & -- Universit\"{a}t zu K\"{o}ln, Germany
\end{tabular}


==> preface.tex <==
%to switch ON running title
%\markboth{Preface}{Preface}

\wstoc{Preface}{}

\title{Preface}

The {\it Tenth International Conference on Recent Progress in
Many-Body Theories} (RPMBT-10) was held at the University of
Washington in Seattle, USA during the period 10-15 September, 1999.
The present volume contains the texts of most of the invited talks
delivered at the conference and a selection from among the many poster
presentations.

The general format and style of the conference followed the accepted
and well-developed pattern for the series, focusing on the
development, refinement and important applications of the techniques
of quantum many-body theory.  The intention of the series has always
been to cover in a broad and balanced fashion both the entire spectrum
of theoretical tools developed to tackle the quantum many-body problem
and their major fields of application.  One of the main aims of the
series is to foster the exchange of ideas and techniques among
physicists working in such diverse areas of applications of many-body
techniques as nuclear and subnuclear physics, astrophysics, atomic and
molecular physics, quantum chemistry, complex systems, quantum field
theory, strongly correlated electronic systems, magnetism, quantum
fluids and condensed matter physics.

Quantum many-body theory as a discipline in its own right dates
largely from the 1950's, and is hence in many senses already a
mature subject.  Despite this apparent maturity the field remains
vibrant and active, vigorous and exciting, vital and important.
Indeed, the successes, importance and vitality of the field have
very clearly been recognized by the sharing of the 1998 Nobel Prizes
in both Physics and Chemistry by the many-body theorists Robert
Laughlin, Walter Kohn and John Pople.  It is a source of great
pleasure to all of us who work in quantum many-body theory that
important achievements in our subject have been thus recognized at
the very highest level.  We were also especially delighted that two
of these then most recent Nobel Laureates, Kohn and Laughlin,
accepted invitations to deliver keynote lectures at RPMBT-10...

A major challenge will be to define and explore these important
areas of overlap in such likely arenas as phase transitions and the
related competing effects of quantum versus thermal fluctuations;
spontaneous symmetry breaking; the unifying role of gauge invariance
(and perhaps other symmetries); concepts from complexity theory,
including the role of correlations and fluctuations in complex
systems, and the competition between analysis and synthesis as modes
of understanding many-body systems; entropy and its generation and
flow; and nonlinearity and its appearance and role at the boundary
between microscopic and mesoscopic descriptions of many-body
systems.  One can perhaps begin to glimpse some insights within the
present proceedings into some of these as areas of future forefront
activity in quantum many-body theory. In this case it may well be
that RPMBT-10 and its immediate successors will later be identified
as the first in the series at which the seeds of the new discourse
between quantum many-body/field theory and statistical physics took
root.

In any event, the Local Organizing and Programme Committees deserve
great thanks in creating a well-run and productive meeting, with an
exciting programme of talks and poster presentations. It is a pleasure
to thank all of them for their hard work, especially Aurel Bulgac who,
as Chairman, has led and guided them throughout.

\vspace*{0.35in}

\noindent
R.F. Bishop \hfill Manchester, U.K.\\
{\itshape (Chairman, International Advisory Committee}
\hfill 31 December 1999\\
{\itshape for the Series of International Conferences on}\\
{\itshape Recent Progress in Many-Body Theories)}


==> proc1.tex <==
%\documentclass{ws-procs961x669}
%\begin{document}

\wstoc{For proceedings editors: Combining contributions\\ using
WS-procs961x669 master document in \LaTeX2e}{F. Author}

\title{For proceedings editors:\\ Combining
contributions using WS-procs961x669\\ master document in \LaTeX2e}

\author{First Author}
\index{author}{Author, F.} % or \aindx{Author, F.}

\address{World Scientific Publishing Co, Production Department,\\
5 Toh Tuck Link, Singapore 596224, \\E-mail: wspc@wspc.com.sg}

\begin{abstract}
ws-procs961x669.tex is the master file to input all the papers from
front matter, body and end matter files.
\end{abstract}

\keywords{Master file; \LaTeX; Proceedings; World Scientific Publishing.}

\section{Master File}
You can obtain these files from the following website:\\
\url{http://www.icpress.co.uk/authors/stylefiles.shtml#conference} and \\
\url{http://www.worldscientific.com/page/authors/proceedings-stylefiles}.

\

All the subdocuments are arranged in this master file in the
following sequence:
\begin{verbatim}
\documentclass{ws-procs961x669}

\usepackage{ws-toc,ws-multind}
\makeindex{author}                    %to invoke author index

\begin{document}
\titlepages
\input preface.tex
\cleardoublepage
\include organizers.tex
\blankpage
\mastertoc
%\part{Part Title}{}                  %optional part title
\include{proc1}
\include{proc2}
%\part{Second Part}{}                 %optional part title
\include{proc3}
\blankpage
\printindex{author}{AUTHOR INDEX}     %to print Author Index
\end{document}
\end{verbatim}

\section{Pagination}

Pages i--iv are always the same and are prepared by the publisher.
The pagination of the rest of the front matter depends on the length
of the various sections (preface, organizing committee's text,
contents). Each front matter section should start on an odd
right-hand page. The following is an example of proceedings
pagination:

\begin{romanlist}[(iii)]

\item Front matter:

\begin{tabular}{@{}lll@{}}
page i &--- & half-title page, prepared by publisher\\
page ii &--- & blank page\\
page iii &--- & full-title page, prepared by publisher\\
page iv &--- & copyright page, prepared by publisher\\
pages v--ix &--- & preface text\\
page xi &--- & organizing committees text\\
pages xiii--xx &--- & contents text (TOC)\\
\end{tabular}\\

The first available front matter page is page v.\\

\item Body text:

\begin{tabular}{@{}lll@{}}
odd page &--- & First article, followed by remaining articles\\
\end{tabular}\\

\item Back matter (optional):

\begin{tabular}{@{}lll@{}}
odd page &--- & participants list\\
\end{tabular}\\

Back matter text must start on an odd page.

\end{romanlist}

\noindent{\bf If the organization of the contributors' manuscripts
is different from the above pagination guidelines, please e-mail the
respective desk-editor for advice.}

\begin{table}
\tbl{This table shows how the author names should appear in running head and TOC depending
upon the number of authors contributing that paper.}
{\begin{tabular}{ll} \toprule
No. of Authors & Author Names\\
\colrule
1 & L. Hatcher\\
2 & I. A. Pedrosa \& I. Guedes\\
3 & B. Feng, X. Gong \& X. Wang\\
4 and more & S. R. Choudhury {\it et al.}\\\botrule
\end{tabular}}
\begin{tabnote}
For TOC and Running Heads, the author names should appear in initial and surname format, e.g. LEE HATCHER should be abbreviated as L.~HATCHER.\\
\end{tabnote}
\end{table}

\section{Running Head}

Preparation of the running head is optional.
Each contribution must have \verb|\markboth| at the preamble to set
the running head.

\verb|\markboth{Author's Name on Even Page}{Article Title on Odd Page}|

\section{Master TOC}

Each contribution must have \verb|\wstoc{#1}{#2}| at the preamble to create
the combined table of contents.

\verb|\wstoc{Article Title}{Author's Name}|

\section{Preparing the Individual Contributions for Combining}

The following highlighted changes should be made in all the contributions provided by the individual contributors before including them in the master document.

\begin{verbatim}
Contribution provided by an        Modified contribution, ready to
individual contributor:            get included in the master
                                   document:

%proc1.tex                         %proc1.tex
\documentclass{ws-procs961x669}     \markboth{A. Author}{Paper title}
\begin{document}                   \wstoc{Paper title}{A. Author}
\title{PAPER TITLE}                \title{Paper title}
\author{A. AUTHOR}                 \author{A. Author}
                                   \aindx{Author, A.}
\address{Institute of ...}         \address{Institute of ...}
\begin{abstract}                   \begin{abstract}
We search for ...                  We search for ...
\end{abstract}                     \end{abstract}
\keywords{Keyword1; ...}           \keywords{Keyword1; ...}
\bodymatter                        \bodymatter
\section{Introduction}             \section{Introduction}
String theory ...                  String theory ...
\begin{thebibliography}{00}        \begin{thebibliography}{00}
\bibitem{t1} A. Sen, ...           \bibitem{t1} A. Sen, ...
\bibitem{t2} P. Horava, ...        \bibitem{t2} P. Horava, ...
...                                ...
\end{thebibliography}              \end{thebibliography}
%for BiBTeX users                  %for BiBTeX users
%\bibliographystyle{ws-pro...}     %\bibliographystyle{ws-pro...}
%\bibliography{sample}             %\bibliography{sample}
\end{document}                     \vfill
                                   \pagebreak
\end{verbatim}

\section{Author Index}

To create an ``author'' index, the following
declarations should be included in the master \TeX{}
file:

\begin{verbatim}
\makeindex{author}      % in the preamble to invoke author index
\printindex{author}{AUTHOR INDEX} % at end to print author index
\end{verbatim}

In text, the author index entries are marked with:

\verb|\index{autor}{entry}| or \verb|\aindx{entry}|

\section{Compiling the Master File in \LaTeX2e}

To complete the job, compile your file as follows:

\begin{enumerate}[(4)]
\item latex ws-procs961x669
\item latex ws-procs961x669
\item bibtex~proc2\hskip48pt{\tt\% Chapters using \btex{} database should}\\
\verb|           |\hskip45pt {\tt \% be compiled individually in `bibtex'.}
\item makeindex author\hskip25pt {\tt \% author index}
\item latex ws-procs961x669
\item latex ws-procs961x669
\end{enumerate}

\begin{thebibliography}{9}
\bibitem{lamp94}
L.~Lamport, \emph{\LaTeX, A Document Preparation System}. (Addison-Wesley,
  Reading, MA, 1994), 2nd edition.
\bibitem{lamp87} L. Lamport, \emph{Make Index: An Index Processor For LaTeX}, (1987).
\end{thebibliography}

%\end{document}


==> proc3.tex <==
%to switch ON running title
%\markboth{L. Hatcher}{Quantum States from Tangent Vectors}

\wstoc{Sample chapter: Quantum states from tangent vectors}{J. M. Isidro}

\title{Sample chapter: Quantum states from tangent
vectors}

\author{Jos\'e M. Isidro}
\aindx{Isidro, J. M.}

\address{Instituto de F\'\i{s}ica Corpuscular (CSIC--UVEG),
Apartado de Correos 22085,\\
Valencia 46071, Spain\\
and\\
Max-Planck-Institut f\"ur Gravitationsphysik,
Albert-Einstein-Institut,\\
D-14476 Golm, Germany\\
\email{jmisidro@ific.uv.es}}

\begin{abstract}
We argue that tangent vectors to classical phase space give rise to
quantum states of the corresponding quantum mechanics. This is
established for the case of complex, finite-dimensional, compact,
classical phase spaces $\mathcal{C}$, by explicitly constructing
Hilbert-space vector bundles over $\mathcal{C}$. We find that these
vector bundles split as the direct sum of two holomorphic vector
bundles: the holomorphic tangent bundle $T(\mathcal{C})$, plus a
complex line bundle $N(\mathcal{C})$. Quantum states (except the
vacuum) appear as tangent vectors to $\mathcal{C}$.  The vacuum state
appears as the fibrewise generator of $N(\mathcal{C})$.  Holomorphic
line bundles $N(\mathcal{C})$ are classified by the elements of ${\rm
Pic}({\cal C})$, the Picard group of $\mathcal{C}$. In this way ${\rm
Pic}({\cal C})$ appears as the parameter space for nonequivalent
vacua. Our analysis is modelled on, but not limited to, the case when
$\mathcal{C}$ is complex projective space ${\bf CP}^n$.
\end{abstract}

\bodymatter

\section{Introduction}\label{intro}
Fibre bundles are powerful tools to formulate the gauge theories of
fundamental interactions and gravity.\cite{LIBAZCA} The question
arises whether or not quantum mechanics may also be formulated
fibre bundles.\footnote{The powerful tools of the gauge theories.}
Important physical motivations call for such a formulation.

In quantum mechanics one aims at constructing a Hilbert-space vector
bundle over classical phase space. In geometric quantisation this
goal is achieved in a two-step process that can be very succinctly
summarised as follows. One first constructs a certain holomorphic
line bundle (the {\it quantum line bundle}\/) over classical phase
space. Next one identifies certain sections of this line bundle as
defining the Hilbert space of quantum states. Alternatively one may
skip the quantum line bundle and consider the one-step process of
directly constructing a Hilbert-space vector bundle over classical
phase space. Associated with this vector bundle there is a principal
bundle whose fibre is the unitary group of Hilbert space.

Standard presentations of quantum mechanics usually deal with the case
when this Hilbert-space vector bundle is trivial. Such is the case,
e.g., when classical phase space is contractible to a point. However,
it seems natural to consider the case of a nontrivial bundle as well.
Beyond a purely mathematical interest, important physical issues that
go by the generic name of {\it dualities}\cite{VAFA} motivate the
study of nontrivial bundles.

Given a certain base manifold and a certain fibre, the trivial bundle
over the given base with the given fibre is unique. This may mislead
one to conclude that quantisation is also unique, or independent of
the observer on classical phase space. In fact the notion of duality
points precisely to the opposite conclusion, i.e.~to the
nonuniqueness of the quantisation procedure and to its dependence on
the observer.\cite{VAFA}

Clearly a framework is required in order to accommodate dualities
within quantum mechanics.\cite{VAFA} Nontrivial Hilbert-space vector
bundles over classical phase space provide one such framework. They
allow for the possibility of having different, nonequivalent
quantisations, as opposed to the uniqueness of the trivial
bundle.\footnote{The framework of the vector bundles.}

\enlargethispage*{6pt}

However, although nontriviality is a necessary condition, it is by no
means sufficient. A flat connection on a nontrivial bundle would still
allow, by parallel transport, to canonically identify the
Hilbert-space fibres above different points on classical phase
space. This identification would depend only on the homotopy class of
the curve joining the basepoints, but not on the curve itself.  Now
flat connections are characterised by {\it constant}\/ transition
functions,\cite{KN} this constant being always the identity in the
case of the trivial bundle.  Hence, in order to accommodate dualities,
we will be looking for {\it nonflat}\/ connections.

First, we want to obtain the
wave functions of a generalized pendulum under time-dependent
gravitation by making use of a unitary transformation and the LR
invariant method. As an example, we consider a generalized pendulum
with\break
exponentially increasing mass and constant gravitation. Second,
we want to present a canonical approach for the generalized
time-dependent pendulum which is based on the use of a time-dependent
canonical transformation and an auxiliary\break
transformation.

\section{Properties of ${\bf CP}^n$ as a Classical Phase
Space \label{cipienne} }
We will consider a classical mechanics whose phase space $\mathcal{C}$
is complex, projective $n$-dimensional space ${\bf CP}^n$.  The
following properties are well known.\cite{KN}

Let $Z^1,\ldots,Z^{n+1}$ denote homogeneous coordinates on ${\bf
CP}^n$.  The chart defined by $Z^k\neq 0$ covers one copy of the open
set $\mathcal{U}_k={\bf C}^n$. On the latter we have the holomorphic
coordinates $z^j_{(k)}=Z^j/Z^k$, $j\neq k$; there are $n+1$ such
coordinate charts. ${\bf CP}^n$ is a K\"ahler manifold with respect
to the Fubini-Study metric. On the~chart $(\mathcal{U}_k, z_{(k)})$
the K\"ahler potential reads
\begin{equation}
K(z^j_{(k)},\bar z^j_{(k)})
=\log\left(1+\sum_{j=1}^n z^j_{(k)}\bar z^j_{(k)}\right)\,.
\label{fubst}
\end{equation}
The singular homology ring $H_*({\bf CP}^n,\mathbb{Z})$ contains the
nonzero subgroups
\begin{equation}
H_{2k}({\bf CP}^n,\mathbb{Z})=\mathbb{Z}\,,\qquad k=0,1,\ldots,n\,,
\label{oncero}
\end{equation}
while
\begin{equation}
H_{2k+1}({\bf CP}^n,\mathbb{Z})=0\,,\qquad k=0,1,\ldots, n-1\,.
\label{oncerox}
\end{equation}
We have ${\bf CP}^{n}={\bf C}^n\cup {\bf CP}^{n-1}$, with ${\bf
CP}^{n-1}$ a hyperplane at infinity. Topologically, ${\bf CP}^{n}$ is
obtained by attaching a (real) $2n$-dimensional cell to ${\bf
CP}^{n-1}$. ${\bf CP}^n$ is simply connected,
\begin{equation}
\pi_1({\bf CP}^n)=0\,,
\label{grfund}
\end{equation}
it is compact, and inherits its complex structure from that on ${\bf
C}^{n+1}$. It can be regarded as the Grassmannian manifold
\begin{equation}
{\bf CP}^n={\rm U}(n+1)/({\rm U}(n)\times {\rm U}(1))
=S^{2n+1}/{\rm U}(1)\,.
\label{facx}
\end{equation}

Let $\tau^{-1}$ denote the {\it tautological bundle}\/ on ${\bf
CP}^n$. We recall that $\tau^{-1}$ is defined as the subbundle of the
trivial bundle ${\bf CP}^n\times {\bf C}^{n+1}$ whose fibre at $p\in
{\bf CP}^n$ is the line in ${\bf C}^{n+1}$ represented by $p$. Then
$\tau^{-1}$ is a holomorphic line bundle over ${\bf CP}^n$.  Its dual,
denoted $\tau$, is called the {\it hyperplane bundle}. For any $l\in
\mathbb{Z}$, the $l$th power $\tau^l$ is also a holomorphic line
bundle over ${\bf CP}^n$. In fact every holomorphic line bundle $L$
over ${\bf CP}^n$ is isomorphic to $\tau^l$ for some $l\in\mathbb{Z}$;
this integer is the first Chern class of $L$.

\subsection{Computation of ${\rm dim}\,H^0({\bf CP}^n,
\mathcal{O}(1))$}
\label{xcompt}
\noindent
Next we present a quantum-mechanical computation of ${\rm
dim}\,H^0({\bf CP}^n,\mathcal{O}(1))$ without resorting to sheaf
cohomology. That is, we compute ${\rm dim}\,\mathcal{H}$ when $l=1$
and prove that it coincides with the right-hand side.

Starting with $\mathcal{C}={\bf CP}^{0}$, i.e.~a point $p$ as
classical phase space, the space of quantum rays must also reduce to a
point. Then the corresponding Hilbert space is $\mathcal{H}_1={\bf
C}$. The only state in $\mathcal{H}_1$ is the vacuum
$|0\rangle_{l=1}$. Henceforth, for brevity, we drop the Picard class
index from the vacuum.

\subsection{Representations}\label{wrepp}
The $(n+1)$-dimensional Hilbert space may be
regarded as a kind of {\it defining representation}, in the sense of
the representation theory of ${\rm SU}(n+1)$ when $n>1$. To make this
statement more precise we observe that one can replace unitary groups
with special unitary groups in Eq.~(\ref{facx}). Comparing our results
with those of Sec.~\ref{cipienne} we conclude that the quantum line
bundle $\mathcal{L}$ now equals $\tau$,
\begin{equation}
\mathcal{L}=\tau\,,
\label{ddttx}
\end{equation}
because $l=1$. This is the smallest value of $l$ that produces a
nontrivial $\mathcal{H}$, gives a one-dimensional
Hilbert space when $l=0$.  So our $\mathcal{H}$ spans an
$(n+1)$-dimensional representation of ${\rm SU}(n+1)$, that we can
identify with the defining representation. There is some ambiguity
here since the dual of the defining representation of ${\rm SU}(n+1)$
is also $(n+1)$-dimensional. This ambiguity is resolved by convening
that the latter is generated by the holomorphic sections of the {\it
dual}\/ quantum line bundle
\begin{equation}
\mathcal{L}^*=\tau^{-1}\,.
\label{ddttxx}
\end{equation}
On the chart $\mathcal{U}_j$, $j=1,\ldots,n+1$, the dual of the
defining representation is the linear span of the covectors
\begin{equation}
\langle (j)0|\,,\qquad  \langle (j)0|A_i(j)\,,\qquad i=1,2,\ldots,n\,.
\label{pannx}
\end{equation}

Taking higher representations is equivalent to considering the
principal \hbox{${\rm SU}(n+1)$}-bundle (associated with the vector
${\bf C}^{n+1}$-bundle) in a representation higher than the defining
one. We will see next that this corresponds to having $l>1$ in our
choice of the line bundle $\tau^l$.

\section{Tangent Vectors as Quantum States}\label{tvqs}
The converse is not true, as exemplified by the vacuum.  Let us
generalise and replace ${\bf CP}^n$ with an arbitrary classical phase
space $\mathcal{C}$. We would like to write,
\begin{equation}
\mathcal{QH}(\mathcal{C})=T(\mathcal{C})\oplus N(\mathcal{C})\,,
\label{adccxj}
\end{equation}
where $N(\mathcal{C})$ is a holomorphic line bundle on $\mathcal{C}$,
whose fibre is generated by the vacuum state, and $T(\mathcal{C})$ is
the holomorphic tangent bundle. Does Eq.~(\ref{adccxj}) hold in
general?

\begin{table}       %Table~1
\tbl{This table gives the QES condition and the number of moving
poles of $\chi$ for each combination of $b_{1}$ and $b^{\prime}_1$
for the Khare--Mandal model.}
{\begin{tabular}{@{}cccccc@{}}
\hline\\
&&&&&\\[-15pt]
Set & $b1$ & $b1'$ & $n=\lambda_{1}-b_{1}-b_{1}'$
& Condition o $M$ & QES Condition \\
& (Rad/s) & (Rad/s) \\[2pt]
\hline\\
&&&&&\\[-15pt]
1 & 1/4 & 1/4 & $\dfrac{M}{2}-\dfrac{1}{2}$
& $M={\rm odd}$, $M\geq 1$ & $M=2n+1$ \\[8pt]
3 & 3/4 & 1/4 & $\dfrac{M}{2}-1$
& $M={\rm even}$, $M\geq 2$ & $M=2n+1$ \\[8pt]
4 & 1/4 & 3/4 & $\dfrac{M}{2}-1$
& $M={\rm even}$, $M\geq 2$ & $M=2n+1$ \\[8pt]
\hline
\end{tabular} \label{tp1}}
\end{table}

The answer is also affirmative provided that
$\mathcal{C}$ is a complex $n$-dimensional, compact, symplectic
manifold, whose complex and symplectic structures are
compatible. Notice that $\mathcal{C}$ is not required to be K\"ahler;
examples of Hermitian but non-K\"ahler spaces are Hopf
manifolds.\cite{KN} Let $\omega$ denote the symplectic form. Then
$\int_\mathcal{C}\omega^n < \infty$ thanks to compactness,
\begin{equation}
\int_\mathcal{C}\omega^n=n+1\,.
\label{chepelotudo}
\end{equation}
Let us cover $\mathcal{C}$ with a {\it finite}\/ set of holomorphic
coordinate charts $(\mathcal{W}_k,w_{(k)})$, \hbox{$k=1,\ldots,r$};
the existence of such an atlas follows from the compactness of
$\mathcal{C}$. We can pick an atlas such that $r$ is minimal;
compactness implies that $r\geq 2$.

From Table~\ref{tp1}, we see that sets~1 and 2 are valid only when $M$ is odd
and sets~3 and 4 are valid only when $M$ is even.

\section{Discussion}\label{dicu}
Quantum mechanics is defined on a Hilbert space of states whose
construction usually assumes a global character on classical phase
space. Under {\it globality}\/ we understand, as explained in
Sec.~\ref{intro}, the property that all coordinate charts on classical
phase space are quantised in the same way.

A novelty of our approach is the local character of the Hilbert space:
there is one on top of each Darboux coordinate chart on classical
phase space.  The patching together of these Hilbert-space fibres on
top of each chart may be global (trivial bundle) or local (nontrivial
bundle). In order to implement duality transformations we need a
nonflat bundle (hence nontrivial). Flatness would allow for a
canonical identification, by means of parallel transport, of the
quantum states belonging to different fibres.

A duality thus arises as the possibility of having two or more,
apparently different\-, quantum-mechanical descriptions of the same
physics. Mathematically, a duality arises as a nonflat, quantum
Hilbert-space bundle over classical phase space. This notion implies
that the concept of a quantum is not absolute, but relative to the
quantum theory used to measure it.\cite{VAFA} That is, duality
expresses the relativity of the concept of a quantum. In particular,
{\it classical}\/ and {\it quantum}\/, for long known to be deeply
related\cite{PERELOMOV} are not necessarily always the same for all
observers on phase space.

\section*{Acknowledgments}
It is a great pleasure to thank J. de Azc\'arraga for encouragement
and support. Technical discussions with U. Bruzzo and
M. Schlichenmaier are gratefully acknowledged. The author thanks
S. Theisen and Max-Planck-Institut f\"ur Gravitationsphysik,\-
Albert-Einstein-Institut, for hospitality.  This work has been
partially supported\- by research grant BFM2002-03681 from Ministerio
de Ciencia y Tecnolog\'\i{a}, by EU FEDER funds, by Fundaci\'on Marina
Bueno and by Deutsche Forschungsgemeinschaft.

\appendix{Appendix}
We can insert an Appendix here and includes equations which are
numbered as Eq.~(\ref{app1}),
\begin{equation}
\frac{4\pi}{3}r_{ij}^3\cdot\frac{4\pi}{3}p_{ij}^3
=\frac{h^3}{4}\,.
\label{app1}
\end{equation}

\subappendix{Subsection of Appendix}
\begin{equation}
 \frac{5\pi}{10}r_{ij}^2\cdot\frac{5\pi}{10}p_{ij}^7
=\frac{h^3}{4}\,.
\label{app2}
\end{equation}

The answer is trivially affirmative when $\mathcal{C}$ is an analytic
submanifold of ${\bf CP}^n$. Such is the case, e.g., of the embedding
of ${\bf CP}^n$ within ${\bf CP}^{n+l}$,
Grassmann manifolds provide another example.

\begin{thebibliography}{00}

%1.
\bibitem{LIBAZCA} J. de Azc\'arraga and J. Izquierdo, {\it Lie Groups,
Lie Algebras, Cohomology and some Applications in Physics} (Cambridge
Univ. Press, 1995).

%2.
\bibitem{VAFA} C. Vafa, hep-th/9702201.

%3.
\bibitem{KN} S. Kobayashi and K. Nomizu, {\it Foundations of
Differential Geometry} (Wiley, 1996).

%4.
\bibitem{MATONE} G. Bertoldi, A. Faraggi and M. Matone, {\it
Class. Quantum Grav.} {\bf 17}, 3965 (2000).

%5.
\bibitem{MINIC} D. Minic and C. Tze, {\it Phys. Rev.} {\bf D68},
061501 (2003); hep-th/0309239; hep-th/0401028; V. Jejjala, D. Minic
anc C. Tze, gr-qc/0406037.

%6.
\bibitem{CARROLL} R. Carroll, quant-ph/0406203.

%7.
\bibitem{MEX} M. Montesinos and G. T. del Castillo, quant-ph/0407051.

%8.
\bibitem{MPLA} J.M. Isidro, {\it Phys. Lett.} {\bf A301}, 210 (2002);
{\it J. Phys. A\/}: {\it Math. Gen.} {\bf 35}, 3305 (2002); {\it
Mod. Phys. Lett.} {\bf A18}, 1975 (2003); {\it ibid.} {\bf A19}, 349
(2004); hep-th/0407161.

%9.
\bibitem{SCHLICHENMAIER} M. Schlichenmaier, Berezin-Toeplitz
quantization and Berezin's symbols for arbitrary compact K\"ahler
manifolds, in {\it Coherent States}, {\it Quantization and Gravity},
eds.~M.~Schlichenmaier {\it et~al.} (Polish Scientific Publishers PWN,
2001).

%10.
\bibitem{LIBSCHL} M. Schlichenmaier, {\it An Introduction to Riemann
Surfaces, Algebraic Curves and Moduli\- Spaces} (Springer, 1989).

%11.
\bibitem{PERELOMOV} A. Perelomov, {\it Generalized Coherent States and
their Applications} (Springer, 1986).
\end{thebibliography}
\vfill
\pagebreak
% http://arxiv.org/pdf/quant-ph/0407159.pdf
